Protectionism and economic growth: Causal evidence from the first era of globalization

We investigate how protectionist policies influence economic growth. Our empirical strategy exploits an extraordinary tax scandal that gave rise to an unexpected change of government in Sweden. A free-trade majority in parliament was overturned by a protectionist majority in 1887. The protectionist government increased tariffs. We employ the synthetic control method to select control countries against which economic growth in Sweden can be compared. We do not find evidence suggesting that protectionist policies influenced economic growth and examine channels why. The new tariff laws increased government revenue. However, the results do not suggest that the protectionist government stimulated the economy by increasing government expenditure.

==> unused_text.tex <==

%\section{The tariff-growth paradox}


%Theories suggest a positive effect of international trade on economic growth. In early growth models (e.g. Harrod-Domar model \citep{Harrod1939, Domar1946}) liberalizing trade increases growth \citep{Srinivasan1999}). In neoclassic growth models (e.g. extended Solow model \citep{Baldwin1992}) or optimal-saving models \citep{SrinivasanBhagwati1980}) liberalizing trade increases growth until the economy converges to its free-trade equilibrium and the growth rate returns to its initial steady-state value. 

%Empirical evidence on the trade-growth nexus is mixed. Trade increased growth in the second half of the 20th century \citep{Dollar1992, SachsWarner1995, Edwards1998, FrankelRomer1999, RodriguezRodrik2000, Dreher2006, Gygli2019}. Similarly, liberalizing trade increased growth while protectionism decreased growth \citep{Krugman1979, Krugman1981, Krugman1990, DixitNorman1980, Ethier1982, Lucas1988, Romer1990, RiveraRomer1991, GrossmanHelpman1991}. 

%Contrary to findings after WW2, early country-specific evidence suggests that trade liberalization slowed down economic growth and protectionism accelerated economic growth in the second half of the 19th century \citep{bairoch1972EER, bairoch1989}. Cross-country studies confirm the 'tariff-growth paradox' \citep{o'rourke2000, ClemensWilliamson2004, Jacks2006}. These studies do not, however, report causal evidence. Endogeneity may result from reverse causality (countries enjoying economic growth may implement protectionist trade policies) and omitted variables (underlying trends may influence economic growth and trade policy). Rather than higher tariffs causing higher growth, the correlation might be driven by outliers. Labor-scarce and land-abundant countries (e.g. Canada and Argentina) relied heavily on customs revenues and enjoyed favorable growth prospects with little link between the two \citep{Irwin2002}.

%The 1870s were a period of synchronized economic depression across a wide set of countries \citep{Solomou1998}. In the post Cobden-Chevalier world, most countries followed a liberal trade regime in the 1860s and 1870s. In response to the "long depression" of the 1870s, some countries raised tariffs. Increasing tariffs coincided with a general economic upswing in the 1880s, explaining much of the correlation between higher tariffs and economic growth. However, growth rates of countries that raised tariffs in the 1870s are not significantly different from growth rates of countries that did not raise tariffs \citep{schularick2011}.

%Studies on average tariffs and growth rates neglect considerable heterogeneity in the tariff structure of countries. Theory suggests that the relationship between trade and growth depends on whether trade promotes resources allocated towards activities that generate long-run growth \citep{GrossmanHelpman1991, RodriguezRodrik2000}. Therefore, tariffs on agricultural commodities may have different effects on growth than tariffs on raw materials, manufactured goods or fiscal tariffs. In the first era of globalization, agricultural tariffs were somewhat negatively correlated with growth and tariffs on manufactured goods were likely growth-enhancing \citep{lehmann2011restat}.\footnote{This evidence is detrimental to findings on the late 20th century, when liberalizing tariffs on imported capital and intermediate goods led to faster growth \citep{EstevadeordalTaylor2013}.} Fiscal tariffs were not correlated with growth during that time \citep{lehmann2011restat}.

%Intentions behind trade policies vary substantially between countries. This is especially true for the second half of the 19th century. The United States followed a protectionist strategy for their manufacturing industry. Many Latin American countries tried to increase government revenues by raising tariffs while France and Germany focused on protecting their agricultural sectors \citep{Tena2010, lehmann2011restat}.

%Cross-country studies do not account for country-specific economic structures. Falling transport costs in the 19th century allowed developing countries to expand their exports of primary products while facing increasing exposure to industrial exports from the relatively well-developed countries of the (Northern) core market \citep{Williamson2006}. Even within well-developed countries, considerable heterogeneity in the economic structure existed and protectionist policies had ambiguous effects on growth \citep{LampeSharp2013}. 





%The DiD estimator constructs the counterfactual using the outcome variable of one control unit or an unweighted average of the outcome variable from the control group. The treatment effect derives from comparing the difference in the outcome variable pre- and post-treatment for the treated unit and the control group. Any macroeconomic shocks or other time effects must affect the treated unit and the control group equally. If additionally the treatment effect on the outcome variable is constant over time, the parallel trends assumption is verified and the DiD estimator measures causal effects. In our case, GDP per capita in Sweden and in our control group would follow parallel trends in the absence of the majority change in the Swedish parliament in 1888.

%The parallel trends assumption is difficult to verify. While it is possible to investigate the pre-treatment trends of the outcome variable, examining trends after treatment is impossible. If the parallel trends assumption is violated, the DiD estimator is biased. We use the synthetic control method relaxes the parallel trends assumption. We measure the synthetic Sweden based on lagged outcome variables (\cite{abadie2019jel}).


%Channels

%Bank assets, the credit volume and the monetary stock decreased substantially after 1887 (Figure \ref{fig: Bank Assets as a Share of GDP}, \ref{fig: Credit as a Share of GDP} and \ref{fig: Monetary Stock as a Share of GDP}). It is conceivable that financial industry's expectations about the future economic prosperity of Sweden gave rise to decreasing bank assets, credit volume and the monetary stock. Uncertainty increased  after the change in government and investors followed a more cautious path. 

%Negative effects of protectionism on the financial industry might have offset positive growth effects through increased government revenues. The financial industry might have anticipated that increased tariffs would raise prices of imported goods which, in turn, may well decrease economic growth.

%\begin{figure}[H]
%	\caption{Bank Assets as a Share of GDP}
%	\begin{center}
%		\includegraphics[width=0.48\textwidth]{graphics/main/synth_by.pdf}
%		\includegraphics[width=0.48\textwidth]{graphics/main/synth_gap_by.pdf}
%       \includegraphics[width=0.48\textwidth]{graphics/main/placebo_nooutlier_by.pdf}
%      \includegraphics[width=0.48\textwidth]{graphics/main/rmspe_by.pdf}
%	\end{center}
%	\footnotesize{\textit{Sources:} \citet{MadsenAng2016}}
%	\label{fig: Bank Assets as a Share of GDP}
%\end{figure}

%\begin{figure}[H]
%	\caption{Credit as a Share of GDP}
%	\begin{center}
%		\includegraphics[width=0.48\textwidth]{graphics/main/synth_cy.pdf}
%		\includegraphics[width=0.48\textwidth]{graphics/main/synth_gap_cy.pdf}
%        \includegraphics[width=0.48\textwidth]{graphics/main/placebo_nooutlier_cy.pdf}
%        \includegraphics[width=0.48\textwidth]{graphics/main/rmspe_cy.pdf}
%	\end{center}
%	\footnotesize{\textit{Sources:} \citet{MadsenAng2016}}
%	\label{fig: Credit as a Share of GDP}
%\end{figure}

%\begin{figure}[H]
%	\caption{Monetary Stock as a Share of GDP}
%	\begin{center}
%		\includegraphics[width=0.48\textwidth]{graphics/main/synth_my.pdf}
%		\includegraphics[width=0.48\textwidth]{graphics/main/synth_gap_my.pdf}
%        \includegraphics[width=0.48\textwidth]{graphics/main/placebo_nooutlier_my.pdf}
%        \includegraphics[width=0.48\textwidth]{graphics/main/rmspe_my.pdf}
%	\end{center}
%	\footnotesize{\textit{Sources:} \citet{MadsenAng2016}}
%	\label{fig: Monetary Stock as a Share of GDP}
%\end{figure}


\section{Sensitivity}
\subsection{GDP}
 Overall, our findings are robust to the "leave-one-out" sensitivity analyses with one exception: Norway is an important control unit; it receives 56.1 percent of the weight when measuring the synthetic Sweden. When excluding Norway, the synthetic Sweden does not follow Sweden's pre-treatment GDP trend well. However, when constructing a synthetic Sweden excluding Norway, we also do not observe that protectionist policies influenced economic growth. 
 
 %We use country classifications of previous studies such as \citet{%kindleberger1951group, mundell1957international, bairoch1972EER, krasner1976state, Capie1983,
%O'Rourke1996, o'rourke2000, Irwin1998, Irwin2002, RodriguezRodrik2000, ClemensWilliamson2004, Williamson2006, %jacks2010trade, %Tena2010, tena2012, 
%schularick2011}.
 
 %An important requirement for SC analyses is that the donor pool of control countries is homogeneous enough \citep{abadie2019jel}. All countries in our donor pool were industrializing during the 1870s and 1880s. Some countries were still monarchies (including Sweden) but clearly transitioning to democracies while others were already parliamentary democracies or direct democracies. Importantly, in all countries in our donor pool citizens or elected representatives of the citizens possessed substantial political power and influenced national policies.
 
 
 
 Hjalmar Branting, the editor of \textit{Tiden} and \textit{Social-Deomkraten} who would become the first social democratic prime minister of Sweden in 1920, complained about the colors of the ballot papers but concurrently admitted that it would not change the overall election results as in the candidates who would represent Stockholm in the \textit{Riksdag}.
 
 
 footnote:  The parliamentarians could have also chosen another free trade government considering the expressed majority for free trade policies. Instead they opted for installing a protectionist government.
 
 
 
 
 While the tariffs brought additional government revenues, they also meant an increase in consumer prices \citep{Bohlin2005}. To offset the price increase, fiscal tariffs were decreased \citep{Haeggqvist2018}. In 1885, the average tariff on non-competing agricultural products\footnote{Non-competing agricultural products were mainly coffee beans, sugar and tobacco.} was 42 percent \citep{Bohlin2005}. From 1888 to 1890, The average tariff on non-competing agricultural products decreased to 17 percent \citep{Bohlin2005}. 

Bildt resigned on 12 October 1889. The protectionist regime was established and Bildt saw his duties fulfilled \citep{Britannica1911}. Gustav Akerhjelm\footnote{Gustav Akerhjelm was a member of the protectionist majority party of the first chamber. The party was found in 1888 and represented protectionist and conservative views.} became the new prime minister and followed the political course set by his predecessor. 



\subsection{Spring and Fall Election 1887}
In 19th century Sweden, protectionists and free traders proposed policies, which were targeted at their individual electorate. Capital owners and workers voted for free traders in both parliamentary elections of 1887 \citep{LehmannVolckart2011}. The largest farmers, which were affected the most by agricultural imports, consistently supported a protectionist policy while smallholders and middling farmers initially voted for free traders \citep{LehmannVolckart2011}. In the 1887 fall election, a majority of all farmers supported protectionists, although small and medium farms mostly specialized in animal husbandry and did not compete with grain imports. \citet{LehmannVolckart2011} attribute this shift in voting behavior to a loss of trust in the liberal government and the influence of protectionist propaganda.



(...) and appendix \ref{sec: Cartoon about O. Larsson} illustrates the surprise and cynical appreciation of the protectionists for Larsson

\section{Cartoon about O. Larsson}
\label{sec: Cartoon about O. Larsson}

\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.75\textwidth]{graphics/main/20200926_cartoon.png}
	\end{center}
\end{figure}

The text reads as follows: \textit{``
The cavalry of the new system gives a farewell parade for its esteemed creator.''}


\footnote{11 kronor and 58 \"{o}re was a small amount. Anecdotal descriptions of the events in fall and winter 1887/88 include a protectionist celebration with a banquet in the restaurant Hasselbacken in Stockholm. It is told that the dinner cost exactly 11 kronor and 58 \"{o}re per guest.}

Data Section:

The dataset from \citet{MadsenAng2016} covers 21 advanced economies since 1870 on an annual basis. It comprises measures for bank assets, credit and monetary stock. Data mostly comes from \citet{mitchel2007international}, \citet{goldsmith1969financial}, and national statistics offices. 

Results Section:


=====================

THOUGHTS ON THE DIRECTION OF THE BIAS.

We are interested in 
\[
\alpha_t=Y_{1t}^{I}-\sum_jw_jY_{jt}^N=Y_{1t}-\sum_jw_jY_{jt}^N
\]
Suppose that there are negative spillovers such that  the observed $Y_{jt}$ is smaller than the potential outcome in the absence of the treatment $Y_{jt}^N$ for $j>1$, i.e.,  $Y_{jt}^N>Y_{jt}$ . Then
\[
\alpha_t=Y_{1t}-\sum_jw_jY_{jt}^N<Y_{1t}-\sum_jw_jY_{jt}
\]
That is, we overestimate the true effect (but not necessarily in terms of the magnitude).

=====================


Negative spill-over effects from Sweden's tariff policy on trade partners may bias our results. Swedish import tariffs may decrease donor pool countries' GDP by decreasing donor pool countries' exports to Sweden. If this is true, synthetic Sweden's GDP would be larger, its difference to Sweden's actual GDP greater in absolute terms (more negative), and the ratio of post- and pre-treatment RMSPE larger. Therefore, we estimate the lower bound of the tariff policy effect's magnitude, which is not to be mistaken with the actual tariff policy effect on Swedish GDP: Following the negative spill-over argument and our inference procedure, the tariff policy should have decreased Sweden's GDP.

We identify the trade partners most affected by Sweden's tariff policy. Bilateral trade flows between countries increase with countries' economic sizes and decrease with distance \citep{isard1954location, anderson1979theoretical, EatonKortum2002, AndersonvanWincoop, Helpmanetal2008}. The gravity model is well established in international trade theory and new evidence corroborates its empirical validity \citep{head2014gravity, andersen_etal2020, Carrere2020}. High gravity countries for Sweden are  If we exclude countries with large export shares 


We define a high gravity county in our study if more than 10 percent of a country's total exports go to Sweden. 


%\footnote{We also investigate whether the Swedish protectionist policies decreased imports from countries which depend on exporting their goods to Sweden. A substantial decrease of exports to Sweden would have likely impacted GDP in these countries. However, Sweden was a minor trade partner for all donor pool countries. Exports to Sweden as a share of total exports did not exceed 15 percent for any donor pool country and were much smaller for most countries.}


\begin{center}{\parbox[b]{16.5cm}{\footnotesize \emph{Notes}: The table shows the results of our estimations on the effect of the 2020 US presidential elections on the expectations of international experts. Expectations are measured regarding four key macroeconomic variables until the year 2023: The growth rate of GDP in \% (Column I), the rate of inflation in \% (Column II), the level of unemployment in \% (Column III), and the level of trade as share of GDP in \% (Column IV). Robust standard errors (adjusted for arbitrary heteroskedasticity) are reported in parentheses. ``Country-FE'' are fixed effect on the country level, ``Dist. Elect. FE'' are fixed effects for the distance (in days) between the time experts filled their survey and the election day, and ``Survey Time'' denoted the duration (in seconds) experts took to fill out their survey.

\vspace{0.2cm}

\begin{tabular}{r l}
***& Significant at the 1 percent level, \\
** & Significant at the 5 percent level, \\
*  & Significant at the 10 percent level \\
\end{tabular}

}} \end{center}\textbf{}
